FSNet: Redesign Self-Supervised MonoDepth for Full-Scale Depth Prediction for Autonomous Driving

Predicting accurate depth with monocular images is important for low-cost robotic applications and autonomous driving. This study proposes a comprehensive self-supervised framework for accurate scale-aware depth prediction on autonomous driving scenes utilizing inter-frame poses obtained from inertial measurements. In particular, we introduce a Full-Scale depth prediction network named FSNet. FSNet contains four important improvements over existing self-supervised models: (1) a multichannel output representation for stable training of depth prediction in driving scenarios, (2) an optical-flow-based mask designed for dynamic object removal, (3) a self-distillation training strategy to augment the training process, and (4) an optimization-based post-processing algorithm in test time, fusing the results from visual odometry. With this framework, robots and vehicles with only one well-calibrated camera can collect sequences of training image frames and camera poses, and infer accurate 3D depths of the environment without extra labeling work or 3D data. Extensive experiments on the KITTI dataset, KITTI-360 dataset and the nuScenes dataset demonstrate the potential of FSNet. More visualizations are presented in \url{https://sites.google.com/view/fsnet/home}

==> secs/image_infer.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{secs/monodepth_infer-crop.pdf}
    \caption{Online inference pipeline of FSNet. Dense full-scale Depth $d_0$ is first predicted from the trained network.  The prediction will be merged with sparse VO points $d_{vo}$ to produce accurate final prediction. The 3D SLIC algorithm is used to segment the image and limit the scale of the post-optimization problem. Only processes within the yellow frame needs to be trained in the training phase.
    }
    \label{fig:monodepth_infer}
\end{figure*}

==> secs/image_init.tex <==
%\begin{figure}
%    \centering
%    \includegraphics[{width=0.35\textwidth}]{secs/monodepth_init_range-crop.pdf}
%    \caption{Using the trained model as the reference, we demonstrate the area with reconstruction error less than 1 pixel. when the initial depth is 15 meters (upper) and 100 meters (lower). These fraction of pixels produce correct gradients at initialization.
    }
%    \label{fig:monodepth_init}
%\end{figure}

==> secs/supsec-0-prove-proportion.tex <==
\section{}

==> secs/table_kitti.tex <==

\begin{table*}[]
\caption{Performance of full-scale MonoDepth on KITTI Eigen Split. For scale factor, "GT" is using LiDAR median scaling methods and "None" means we directly evaluate the error without post-processing scale. "\textbf{*}" indicates methods using sequential images in test time. }
    \label{tab:kitti_test}
    \centering
    \begin{tabular*}{0.91\textwidth}{|l|c|c|c|c|c|c|c|c|}
    \hline {\bf Methods} & {\bf Scale Fac.} &  \cellcolor{red!25}{Abs Rel$\downarrow$} & \cellcolor{red!25}{Sq Rel$\downarrow$} & \cellcolor{red!25}{\bf RMSE$\downarrow$} & \cellcolor{red!25}{RMSE log$\downarrow$} & \cellcolor{blue!25}{$\delta<1.25$ $\uparrow$} & \cellcolor{blue!25}{$\delta<1.25^2$ $\uparrow$} & \cellcolor{blue!25}{$\delta<1.25^3$ $\uparrow$} \\ 
    \hline
    MonoDepth \cite{monodepth2} & GT  &   0.116  &   0.903  &   4.863  &   0.193  &   0.877  &   0.959  &   0.981  \\
     DNet \cite{xue2020toward} &  GT &  0.113  &   0.864  &   4.812  &   0.191  &   0.877  &   0.960  &   0.981  \\
    % MultiChannel (FSNet) & GT &  0.117  &   0.895  &   4.762  &   0.191  &   0.872  &   0.959  &   0.982  \\
    %  + Optical Flow (FSNet) &  GT & 0.117  &   0.881  &   4.746  &   0.191  &   0.873  &   0.959  &   0.981  \\
     \textbf{FSNet (single frame)} & GT  &   \textbf{0.113}  &   \textbf{0.857}  &   \textbf{4.623}  &   \textbf{0.189}  &   \textbf{0.876} &   \textbf{0.960}  &   \textbf{0.982}  \\
      \textbf{*FSNet (post-opt)}  & GT  & \textbf{0.111}  &   \textbf{0.829}  &   \textbf{4.393}  &   \textbf{0.185}  &   \textbf{0.883}  &   \textbf{0.961}  &   \textbf{0.983}  \\
    \hline
     DNet \cite{xue2020toward} & None &  0.118  &   0.925  &   4.918  &   0.199  &   0.862  &   0.953  &   0.979 \\
    % MultiChannel (FSNet) & None &   0.123  &   0.936  &   4.910  &   0.202  &   0.857  &   0.954  &   0.980  \\
    %+ Optical Flow (FSNet) &  None &  0.118  &   0.924  &   4.861  &   0.200  &   0.860  &   0.955  &   0.980  \\
       \textbf{FSNet (single frame)} &  None  & \textbf{0.116}  &   \textbf{0.923}  &   \textbf{4.694}  &   \textbf{0.194}  &   \textbf{0.871}  &   \textbf{0.958}  &   \textbf{0.981}  \\
       \textbf{*FSNet (post-opt)}   & None  & \textbf{0.109}  &   \textbf{0.866}  &   \textbf{4.450}  &   \textbf{0.189}  &   \textbf{0.879}  &   \textbf{0.959}  &   \textbf{0.982}  \\
      \hline
    \end{tabular*}
    
\end{table*}
